TOM-Net: Learning Transparent Object Matting from a Single Image

This paper addresses the problem of transparent object matting. Existing image matting approaches for transparent objects often require tedious capturing procedures and long processing time, which limit their practical use. In this paper, we first formulate transparent object matting as a refractive flow estimation problem. We then propose a deep learning framework, called TOM-Net, for learning the refractive flow. Our framework comprises two parts, namely a multi-scale encoder-decoder network for producing a coarse prediction, and a residual network for refinement. At test time, TOM-Net takes a single image as input, and outputs a matte (consisting of an object mask, an attenuation mask and a refractive flow field) in a fast feed-forward pass. As no off-the-shelf dataset is available for transparent object matting, we create a large-scale synthetic dataset consisting of 158K images of transparent objects rendered in front of images sampled from the Microsoft COCO dataset. We also collect a real dataset consisting of 876 samples using 14 transparent objects and 60 background images. Promising experimental results have been achieved on both synthetic and real data, which clearly demonstrate the effectiveness of our approach.

==> figures/real_qual.tex <==
\begin{figure*} \centering
    \makebox[0.12\textwidth]{\footnotesize Background} 
    \makebox[0.12\textwidth]{\footnotesize Input} 
    \makebox[0.12\textwidth]{\footnotesize Rec. Image} 
    \makebox[0.12\textwidth]{\footnotesize Rec. Error} 
    \makebox[0.12\textwidth]{\footnotesize Ref. Flow} 
    \makebox[0.12\textwidth]{\footnotesize Obj. Mask} 
    \makebox[0.12\textwidth]{\footnotesize Att. Mask} 
    \makebox[0.12\textwidth]{\footnotesize Composite} 
    \\
    \raisebox{0.5\height}{\rotatebox{90}{\scriptsize (a) Glass}}
    \includegraphics[width=0.117\textwidth]{images/Results/real/single_still/{1_multi_bg_1.00_1.0_0_ref}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/single_still/{1_multi_bg_1.00_1.0_6_tar}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/single_still/{1_multi_bg_1.00_1.0_5_final_r}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/single_still/{1_multi_bg_1.00_1.0_7_PSNR_27.60_SSIM_0.95_diff}.png}
    \raisebox{0.3\height}{\rotatebox{90}{\tiny P = 27.6, S = 0.95}}
    \includegraphics[width=0.117\textwidth]{images/Results/real/single_still/{1_multi_bg_1.00_1.0_1_fcolor_r}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/single_still/{1_multi_bg_1.00_1.0_3_mask_r}.png}
    \includegraphics[width=0.117\textwidth]{images/Results/real/single_still/{1_multi_bg_1.00_1.0_4_rho_r}.png}
    \includegraphics[width=0.117\textwidth]{images/Results/real/single_still/{1_multi_bg_1.00_1.0_7_transfer_34}.jpg}
    \\
    \raisebox{0.1\height}{\rotatebox{90}{\scriptsize (b) Glass \& Water}}
    \includegraphics[width=0.117\textwidth]{images/Results/real/water/{1_water_1.00_1.0_0_ref}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/water/{1_water_1.00_1.0_6_tar}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/water/{1_water_1.00_1.0_5_final_r}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/water/{1_water_1.00_1.0_7_PSNR_27.32_SSIM_0.95_diff}.png}
    \raisebox{0.3\height}{\rotatebox{90}{\tiny P = 27.3, S = 0.95}}
    \includegraphics[width=0.117\textwidth]{images/Results/real/water/{1_water_1.00_1.0_1_fcolor_r}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/water/{1_water_1.00_1.0_3_mask_r}.png}
    \includegraphics[width=0.117\textwidth]{images/Results/real/water/{1_water_1.00_1.0_4_rho_r}.png}
    \includegraphics[width=0.117\textwidth]{images/Results/real/water/{1_water_1.00_1.0_7_transfer_7}.jpg}
    \\
    \raisebox{0.5\height}{\rotatebox{90}{\scriptsize (c) Lens}}
    \includegraphics[width=0.117\textwidth]{images/Results/real/lens/{1_lens_1.00_1.0_0_ref}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/lens/{1_lens_1.00_1.0_6_tar}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/lens/{1_lens_1.00_1.0_5_final_r}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/lens/{1_lens_1.00_1.0_7_PSNR_27.15_SSIM_0.91_diff}.png}
    \raisebox{0.3\height}{\rotatebox{90}{\tiny P = 27.2, S = 0.91}}   
    \includegraphics[width=0.117\textwidth]{images/Results/real/lens/{1_lens_1.00_1.0_1_fcolor_r}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/lens/{1_lens_1.00_1.0_3_mask_r}.png}
    \includegraphics[width=0.117\textwidth]{images/Results/real/lens/{1_lens_1.00_1.0_4_rho_r}.png}
    \includegraphics[width=0.117\textwidth]{images/Results/real/lens/{1_lens_1.00_1.0_7_transfer_20}.jpg}
    \\
    \raisebox{0.1\height}{\rotatebox{90}{\scriptsize (d) Multi-objects}}
    \includegraphics[width=0.117\textwidth]{images/Results/real/multi/{1_multi1_1.00_1.0_0_ref}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/multi/{1_multi1_1.00_1.0_6_tar}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/multi/{1_multi1_1.00_1.0_5_final_r}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/multi/{1_multi1_1.00_1.0_7_PSNR_25.37_SSIM_0.93_diff}.png}
    \raisebox{0.3\height}{\rotatebox{90}{\tiny P = 25.37, S = 0.93}}
    \includegraphics[width=0.117\textwidth]{images/Results/real/multi/{1_multi1_1.00_1.0_1_fcolor_r}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/multi/{1_multi1_1.00_1.0_3_mask_r}.png}
    \includegraphics[width=0.117\textwidth]{images/Results/real/multi/{1_multi1_1.00_1.0_4_rho_r}.png}
    \includegraphics[width=0.117\textwidth]{images/Results/real/multi/{1_multi1_1.00_1.0_7_transfer_0}.jpg}
    \\
    \raisebox{0.1\height}{\rotatebox{90}{\scriptsize (e) Complex Bull}}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{1_bull_1.00_1.0_0_ref}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{1_bull_1.00_1.0_6_tar}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{1_bull_1.00_1.0_5_final_r}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{1_bull_1.00_1.0_7_PSNR_20.31_SSIM_0.84_diff}.png}
    \raisebox{0.3\height}{\rotatebox{90}{\tiny P = 20.31, S = 0.84}}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{1_bull_1.00_1.0_1_fcolor_r}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{1_bull_1.00_1.0_3_mask_r}.png}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{1_bull_1.00_1.0_4_rho_r}.png}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{1_bull_1.00_1.0_7_transfer_33}.jpg}
    \\                                                                          
    \raisebox{0.\height}{\rotatebox{90}{\scriptsize (f) Complex Dragon}}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{2_dragon_1.00_1.0_0_ref}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{2_dragon_1.00_1.0_6_tar}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{2_dragon_1.00_1.0_5_final_r}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{2_dragon_1.00_1.0_7_PSNR_18.46_SSIM_0.80_diff}.png}
    \raisebox{0.3\height}{\rotatebox{90}{\tiny P = 18.46, S = 0.80}}                   
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{2_dragon_1.00_1.0_1_fcolor_r}.jpg}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{2_dragon_1.00_1.0_3_mask_r}.png}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{2_dragon_1.00_1.0_4_rho_r}.png}
    \includegraphics[width=0.117\textwidth]{images/Results/real/cplx/{2_dragon_1.00_1.0_7_transfer_34}.jpg}
    \\
    \caption{Qualitative results on real data. The PSNR and SSIM between input photographs and reconstructed images are shown right after the error maps. The last column shows the composites on novel backgrounds given the estimated matte. (Best viewed in PDF with zoom.)} \label{fig:real_qualitative}
\end{figure*}


==> figures/refine_vis.tex <==
\begin{figure} \centering
    \makebox[0.09\textwidth]{\footnotesize Input} 
    \makebox[0.09\textwidth]{\footnotesize Coarse Flow} 
    \makebox[0.09\textwidth]{\footnotesize Refined Flow} 
    \makebox[0.09\textwidth]{\footnotesize Coarse Att.} 
    \makebox[0.09\textwidth]{\footnotesize Refined Att.} 
    \\
    \includegraphics[width=0.090\textwidth]{images/Results/refine/{7_water5_0.90__6_tar}.jpg}
    \includegraphics[width=0.090\textwidth]{images/Results/refine/{7_combine_flow}.jpg}
    \includegraphics[width=0.090\textwidth]{images/Results/refine/{7_combine_r_flow}.jpg}
    \includegraphics[width=0.090\textwidth]{images/Results/refine/{7_combine_rho}.jpg}
    \includegraphics[width=0.090\textwidth]{images/Results/refine/{7_combine_r_rho}.jpg}
    \\
    \includegraphics[width=0.090\textwidth]{images/Results/refine/{5_multi2_1.00__6_tar}.jpg}
    \includegraphics[width=0.090\textwidth]{images/Results/refine/{5_combine_flow}.jpg}
    \includegraphics[width=0.090\textwidth]{images/Results/refine/{5_combine_r_flow}.jpg}
    \includegraphics[width=0.090\textwidth]{images/Results/refine/{5_combine_rho}.jpg}
    \includegraphics[width=0.090\textwidth]{images/Results/refine/{5_combine_r_rho}.jpg}
    \\
    \caption{Visualization of the effectiveness of the refinement stage on real data. After refinement, the refractive flow and attenuation mask have more clear structural details (e.g., glass mouth).} \label{fig:refine}
\end{figure}




==> figures/syn_data_samples.tex <==
\begin{figure} \centering
     \makebox[0.075\textwidth]{\footnotesize Bg} 
     \makebox[0.075\textwidth]{\footnotesize Image} 
     \makebox[0.075\textwidth]{\footnotesize Flow Vis} 
     \makebox[0.075\textwidth]{\footnotesize Ref. Flow} 
     \makebox[0.075\textwidth]{\footnotesize Obj. Mask} 
     \makebox[0.075\textwidth]{\footnotesize Att. Mask} 
     \\
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0033_sor1_0066__0000_COCO_val2014_000000366529_ref}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0033_sor1_0066__0000_COCO_val2014_000000366529}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0033_sor1_0066__0000_COCO_val2014_000000366529_cores}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0033_sor1_0066__0000_COCO_val2014_000000366529_flow}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0033_sor1_0066__0000_COCO_val2014_000000366529_mask}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0033_sor1_0066__0000_COCO_val2014_000000366529_rho}
     \\
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0020_piecew1_water18141_0000_COCO_test2015_000000391594_ref}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0020_piecew1_water18141_0000_COCO_test2015_000000391594}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0020_piecew1_water18141_0000_COCO_test2015_000000391594_cores}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0020_piecew1_water18141_0000_COCO_test2015_000000391594_flow}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0020_piecew1_water18141_0000_COCO_test2015_000000391594_mask}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0020_piecew1_water18141_0000_COCO_test2015_000000391594_rho}
     \\
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0163_lens1_0663__0000_COCO_val2014_000000391596_ref}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0163_lens1_0663__0000_COCO_val2014_000000391596}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0163_lens1_0663__0000_COCO_val2014_000000391596_cores}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0163_lens1_0663__0000_COCO_val2014_000000391596_flow}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0163_lens1_0663__0000_COCO_val2014_000000391596_mask}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0163_lens1_0663__0000_COCO_val2014_000000391596_rho}
     \\
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0042_cplx3_0893__0000_COCO_val2014_000000028826_ref}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0042_cplx3_0893__0000_COCO_val2014_000000028826}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0042_cplx3_0893__0000_COCO_val2014_000000028826_cores}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0042_cplx3_0893__0000_COCO_val2014_000000028826_flow}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0042_cplx3_0893__0000_COCO_val2014_000000028826_mask}
     \includegraphics[width=0.075\textwidth]{images/Datasets/render_gt/shape0042_cplx3_0893__0000_COCO_val2014_000000028826_rho}
     \\
    \caption{Examples of synthetic data. Up to down: examples of glass shape, glass with water, lens and complex shape, respectively. First three columns: background images, rendered images, visualization of some refractive flow. Last three columns: ground truth refractive flow field, object mask, attenuation mask. (Best viewed in PDF with zoom.)} \label{fig:rendered_data}
\end{figure}




==> figures/syn_qual.tex <==
\begin{figure*} \centering
    \makebox[0.095\textwidth]{\footnotesize Background} 
    \makebox[0.095\textwidth]{\footnotesize Input} 
    \makebox[0.095\textwidth]{\footnotesize Rec. Image} 
    \makebox[0.095\textwidth]{\footnotesize Rec. Error} 
    \makebox[0.19\textwidth]{\footnotesize Refractive Flow (GT / Est.)} 
    \makebox[0.19\textwidth]{\footnotesize Object Mask (GT / Est.)} 
    \makebox[0.19\textwidth]{\footnotesize Attenuation Mask (GT / Est.)} 
    \\
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/179_shape0028_sor4_0356__0000_COCO_val2014_000000478055_ref.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/179_shape0028_sor4_0356__0000_COCO_val2014_000000478055_tar.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/179_shape0028_sor4_0356__0000_COCO_val2014_000000478055_pred.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/179_shape0028_sor4_0356__0000_COCO_val2014_000000478055_diff.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/179_shape0028_sor4_0356__0000_COCO_val2014_000000478055_gt_fcolor.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/179_shape0028_sor4_0356__0000_COCO_val2014_000000478055_fcolor.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/179_shape0028_sor4_0356__0000_COCO_val2014_000000478055_gt_mask}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/179_shape0028_sor4_0356__0000_COCO_val2014_000000478055_mask.png}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/179_shape0028_sor4_0356__0000_COCO_val2014_000000478055_gt_rho}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/179_shape0028_sor4_0356__0000_COCO_val2014_000000478055_rho.png}
    \\
    \vspace{-0.5em}\makebox[0.38\textwidth]{\scriptsize (a) Glass, I-MSE = $0.21 \times 10^{-2}$} 
    \makebox[0.19\textwidth]{\scriptsize F-EPE = 2.6 / 15.0} 
    \makebox[0.19\textwidth]{\scriptsize M-IoU = 0.99} 
    \makebox[0.19\textwidth]{\scriptsize A-MSE = $0.16 \times 10^{-2}$} 
    \\
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/63_shape0012_sor2_water0125__0000_COCO_val2014_000000408989_ref.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/63_shape0012_sor2_water0125__0000_COCO_val2014_000000408989_tar.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/63_shape0012_sor2_water0125__0000_COCO_val2014_000000408989_pred.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/{63_shape0012_sor2_water0125__0000_COCO_val2014_000000408989_PSNR_29.23_SSIM_0.941_diff}.png}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/63_shape0012_sor2_water0125__0000_COCO_val2014_000000408989_gt_fcolor.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/63_shape0012_sor2_water0125__0000_COCO_val2014_000000408989_fcolor.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/63_shape0012_sor2_water0125__0000_COCO_val2014_000000408989_gt_mask}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/63_shape0012_sor2_water0125__0000_COCO_val2014_000000408989_mask.png}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/63_shape0012_sor2_water0125__0000_COCO_val2014_000000408989_gt_rho}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/63_shape0012_sor2_water0125__0000_COCO_val2014_000000408989_rho.png}
    \\
    \vspace{-0.5em}\makebox[0.38\textwidth]{\scriptsize (b) Glass with Water, I-MSE = $0.15\times 10^{-2}$} 
    \makebox[0.19\textwidth]{\scriptsize F-EPE = 3.8 / 25.0} 
    \makebox[0.19\textwidth]{\scriptsize M-IoU = 0.97} 
    \makebox[0.19\textwidth]{\scriptsize A-MSE = 0.40 $\times 10^{-2}$} 
    \\
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/15_shape0014_lens1_0514__0000_COCO_val2014_000000449828_ref.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/15_shape0014_lens1_0514__0000_COCO_val2014_000000449828_tar.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/15_shape0014_lens1_0514__0000_COCO_val2014_000000449828_pred.jpg}
   \includegraphics[width=0.095\textwidth]{images/Results/synthetic/{15_shape0014_lens1_0514__0000_COCO_val2014_000000449828_PSNR_31.01_SSIM_0.92_}.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/15_shape0014_lens1_0514__0000_COCO_val2014_000000449828_gt_fcolor.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/15_shape0014_lens1_0514__0000_COCO_val2014_000000449828_fcolor.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/15_shape0014_lens1_0514__0000_COCO_val2014_000000449828_gt_mask}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/15_shape0014_lens1_0514__0000_COCO_val2014_000000449828_mask.png}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/15_shape0014_lens1_0514__0000_COCO_val2014_000000449828_gt_rho}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/15_shape0014_lens1_0514__0000_COCO_val2014_000000449828_rho.png}
    \\
    \vspace{-0.5em}\makebox[0.38\textwidth]{\scriptsize (c) Lens, I-MSE = $0.079\times 10^{-2}$}
    \makebox[0.19\textwidth]{\scriptsize F-EPE = 1.5 / 3.7} 
    \makebox[0.19\textwidth]{\scriptsize M-IoU = 1.00} 
    \makebox[0.19\textwidth]{\scriptsize A-MSE = $0.17\times 10^{-2}$} 
    \\
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/1_dog__0000_gradient_7152_ref.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/1_dog__0000_gradient_7152_tar.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/1_dog__0000_gradient_7152_pred.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/1_dog__0000_gradient_7152_diff.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/1_dog__0000_gradient_7152_gt_fcolor.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/1_dog__0000_gradient_7152_fcolor.jpg}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/1_dog__0000_gradient_7152_gt_mask}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/1_dog__0000_gradient_7152_mask.png}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/1_dog__0000_gradient_7152_gt_rho}
    \includegraphics[width=0.095\textwidth]{images/Results/synthetic/1_dog__0000_gradient_7152_rho.png}
    \\
    \vspace{-0.5em}\makebox[0.38\textwidth]{\scriptsize (d) Complex Dog, I-MSE = $0.28\times 10^{-2}$} 
    \makebox[0.19\textwidth]{\scriptsize F-EPE = 5.05 / 40.6} 
    \makebox[0.19\textwidth]{\scriptsize M-IoU = 0.96} 
    \makebox[0.19\textwidth]{\scriptsize A-MSE = $0.16\times 10^{-2}$} 
    \caption{Qualitative results on synthetic data. The first to the fourth columns show background, input image, reconstructed image, and reconstruction error map, respectively. Quantitative results are shown below each example. Dark region in GT flow indicates no valid flow. (Best viewed in PDF with zoom.)} \label{fig:qual_synth}
\end{figure*}


==> tables/real_quant.tex <==
\begin{table}
    \centering
    \caption{Quantitative results on real data.}
    \resizebox{0.48\textwidth}{!}{ 
    \huge
    \begin{tabular}{c|*{2}{c}|*{2}{c}|*{2}{c}|*{2}{c}|*{2}{c}}
        \toprule
        \multirow{2}{*}{} & \multicolumn{2}{c}{Glass} 
                          & \multicolumn{2}{c}{G \& W} 
                          & \multicolumn{2}{c}{Lens} 
                          & \multicolumn{2}{c}{Cplx} 
                          & \multicolumn{2}{c}{Avg} \\
        & PSNR & SSIM  & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\
        \midrule
        Background    & 22.05 & 0.894 & 20.75 & 0.886 & 18.60 & 0.860 & 16.85 & 0.816 & 19.56 & 0.864 \\ 
        CoarseNet     & 25.09 & 0.921 & 23.53 & 0.911 & 21.13 & 0.895 & 17.89 & 0.835 & 21.91 & 0.891  \\ 
        TOM-Net        & 25.06 & 0.920 & 23.53 & 0.911 & 20.89 & 0.893 & 17.88 & 0.835 & 21.84 & 0.890 \\ 
        %\midrule
        %TOMNET(P)     & 25.18 & 0.921  & 23.64 & 0.911 & 20.93 & 0.894 & 17.92 & 0.835 &21.92 & 0.890  \\ 
        \bottomrule
    \end{tabular}
    }
    \label{tab:real_quant}
\end{table}



==> tables/syn_quant.tex <==
\begin{table*} \centering
    \caption{Quantitative results on the synthetic validation set. (The first value for EPE is measured on the whole image and the second measured within the object region. A-MSE and I-MSE are computed on the whole image.)}
    \begin{minipage}{0.93\textwidth}
    \resizebox{\textwidth}{!}{
    \Huge
        \begin{tabular}{c|*{4}{c}|*{4}{c}|*{4}{c}|*{4}{c}|*{4}{c}}
        \toprule
        \multirow{2}{*}{} & \multicolumn{4}{c}{Glass} 
                               & \multicolumn{4}{c}{Glass with Water} 
                               & \multicolumn{4}{c}{Lens} 
                               & \multicolumn{4}{c}{Complex Shape}  
                               & \multicolumn{4}{c}{Average}  \\
                               & \cellcolor{red!25} F-EPE & \cellcolor{red!25}A-MSE & \cellcolor{red!25}I-MSE & \cellcolor{blue!25} M-IoU 
                               & \cellcolor{red!25} F-EPE & \cellcolor{red!25}A-MSE & \cellcolor{red!25}I-MSE & \cellcolor{blue!25} M-IoU 
                               & \cellcolor{red!25} F-EPE & \cellcolor{red!25}A-MSE & \cellcolor{red!25}I-MSE & \cellcolor{blue!25} M-IoU 
                               & \cellcolor{red!25} F-EPE & \cellcolor{red!25}A-MSE & \cellcolor{red!25}I-MSE & \cellcolor{blue!25} M-IoU 
                               & \cellcolor{red!25} F-EPE & \cellcolor{red!25}A-MSE & \cellcolor{red!25}I-MSE & \cellcolor{blue!25} M-IoU \\
        \midrule
        Background    & 3.6 / 30.3 & 1.33 & 0.48 & 0.12 & 6.4 / 53.2 & 1.54 & 0.68 & 0.12 & 10.3 / 39.2 & 1.94 & 1.57 & 0.24 & 6.8 / 56.8 & 2.50 & 0.85 & 0.11 & 6.8 / 44.9 & 1.83 & 0.90 & 0.15 \\
        CoarseNet     & 2.1 / 15.8 & 0.22 & 0.14 & 0.97 & 3.1 / 23.5 & 0.31 & 0.23 & 0.97 & 2.0 / 6.7   & 0.17 & 0.28 & 0.99 & 4.5 / 34.4 & 0.38 & 0.33 & 0.92 & 2.9 / 20.1 & 0.27 & 0.24 & 0.96 \\
        \midrule
        TOM-Net       & 1.9 / 14.7 & 0.21 & 0.14 & 0.97 & 2.9 / 21.8 & 0.30 & 0.22 & 0.97 & 1.9 / 6.6   & 0.15 & 0.29 & 0.99 & 4.1 / 31.5 & 0.37 & 0.32 & 0.92 & 2.7 / 18.6 & 0.26 & 0.24 & 0.96 \\
        \bottomrule
    \end{tabular}
    }
    \end{minipage}
    \hspace{-0.6em}
    \begin{minipage}{0.06\textwidth}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{cc}
            \midrule
            MSE ($\cdot10^{-2}$) \\
            \cellcolor{red!25} $\downarrow$ better \\ 
            \cellcolor{blue!25} $\uparrow$ better\\
            \midrule
        \end{tabular}
        }
    \end{minipage}
    \label{tab:quant_synth}
\end{table*}




==> tables/syn_selfcompare.tex <==
\begin{table}
    \centering
    \caption{Ablation study results. F, A, I, and M are short for flow, attenuation, image reconstruction, and object mask, respectively. (The first value for EPE is measured on the whole image and the second measured within the object region. A-MSE and I-MSE are computed on the whole image.)
    }
    %\Large
    \begin{minipage}{0.41\textwidth}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{*{6}{>{\Large}c}}
        \toprule
        ID & Model Variants & \cellcolor{red!25}F-EPE  & \cellcolor{red!25}A-MSE & \cellcolor{red!25}I-MSE &  \cellcolor{blue!25}M-IoU \\ 
        \midrule
        0 & Background                         & 6.5 / 41.0 & 1.58 & 0.87 & 0.15 \\
        1 & CoarseNet - ($\mathcal{L}^c_{fr}$) & 3.9 / 26.5 & 0.24 & 0.23 & 0.98 \\
        2 & CoarseNet - ($\mathcal{L}^c_{ir}$) & 2.3 / 15.7 & 0.25 & 0.22 & 0.98 \\
        3 & CoarseNet - (multi-scale)          & 2.4 / 16.6 & 0.69 & 0.25 & 0.94 \\
        4 & CoarseNet - (cross-link)           & 2.5 / 17.2 & 0.30 & 0.21 & 0.97  \\
        5 & CoarseNet                          & \textbf{2.2 / 15.4} & 0.28 & 0.18 & 0.97 \\
        \midrule
        6 & CoarseNet + RefineNet              & 2.0 / 13.7 & 0.25 & 0.19 & 0.97 \\
        \bottomrule
    \end{tabular}
    }
    \end{minipage}
    \hspace{-0.7em}
    \begin{minipage}{0.06\textwidth}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccc}
        \midrule
        MSE ($\cdot10^{-2}$) \\ \cellcolor{red!25} $\downarrow$ better \\ \cellcolor{blue!25} $\uparrow$ better \\
        \midrule
    \end{tabular}
    }
    \end{minipage}
    \label{tab:self_compare}
\end{table}



==> tables/user_study.tex <==
% \begin{table}
%     \centering
%     \caption{User Study Results}
%     \begin{tabular}{c*{2}{c}}
%         \toprule
%         Prediction & Real Images & TOMNet  \\
%         \midrule
%         Voting & & \\ 
%         \bottomrule
%     \end{tabular}
%     \label{tab:user_study}
% \end{table}

\begin{table} \centering
% \renewcommand{\arraystretch}{1.5}
% \setlength{\tabcolsep}{.15em}
% \small
    \caption{User study results.}
    \huge
    \resizebox{0.48\textwidth}{!}{
        \begin{tabular}{c|*{3}{c}|*{3}{c}|*{3}{c}|*{3}{c}|*{3}{c}}
        \toprule
        \multirow{2}{*}{} & \multicolumn{3}{c}{Glass} 
                               & \multicolumn{3}{c}{G \& W} 
                               & \multicolumn{3}{c}{Lens} 
                               & \multicolumn{3}{c}{Cplx}  
                               & \multicolumn{3}{c}{All}  \\
                               & P & C & N 
                               & P & C & N
                               & P & C & N 
                               & P & C & N 
                               & P & C & N \\
        \midrule
        Photographs        & 522 & 275 & 31 & 163 & 97 & 16 & 74 & 48 & 16 & 91 & 35 & 12 & 850 & 455 & 75 \\
        Composites    & 531 & 266 & 31 & 145 & 113 & 18 & 73 & 52 & 13 & 78 & 51 & 9 & 827 & 482 & 71 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:user_study}
\end{table}


